A Comprehensive Evaluation of Multi-task Learning and Multi-task Pre-training on EHR Time-series Data

Multi-task learning (MTL) is a machine learning technique aiming to improve model performance by leveraging information across many tasks. It has been used extensively on various data modalities, including electronic health record (EHR) data. However, despite significant use on EHR data, there has been little systematic investigation of the utility of MTL across the diverse set of possible tasks and training schemes of interest in healthcare. In this work, we examine MTL across a battery of tasks on EHR time-series data. We find that while MTL does suffer from common negative transfer, we can realize significant gains via MTL pre-training combined with single-task fine-tuning. We demonstrate that these gains can be achieved in a task-independent manner and offer not only minor improvements under traditional learning, but also notable gains in a few-shot learning context, thereby suggesting this could be a scalable vehicle to offer improved performance in important healthcare contexts.

==> intro_old.tex <==

% To the best of our knowledge,  machine learning for health lacks a full, nuanced analysis of the efficacy of MTL on clinical data and the extent of the possible drawbacks of MTL. Given that health data is notoriously noisy, sparse, and suffers from significant domain shift, this lack of understanding of MTL, one possible tool to help surmount exactly these difficulties, is a serious problem.


% Machine learning for health is a rapidly growing field, attracting significant attention both from industry and academia \todo{cite}. Commensurate with this growing interest is the knowledge that clinical data is fundamentally \emph{different} than general domain data. Clinical data is often smaller, higher-dimensional, and noisier than general domain data, and tasks are more narrowly defined and susceptible to confounders that vary across institutions and demographics \todo{cite} \cite{rajkomar2018scalable, gong2017predicting, Obermeyer447}. These data difficulties impose significant hurdles to effective learning in this domain, and one way people have tried to surmount these obstacles is through multi-task learning (MTL), a machine learning technique in which a model is trained to simultaneously predict several tasks at once in hopes of improving performance without incurring~\emph{negative transfer}, when the introduction of auxiliary tasks harms performance on the tasks of interest.

% MTL has been used extensively in the general domain, where researchers have found both empirical successes~\cite{luong2015multi,zhang2017survey,zhang2018learning}, and theoretical support to argue that MTL can offer performance benefits for sufficiently aligned tasks, while incurring \emph{negative transfer} for insufficiently related tasks~\cite{ndirango2019generalization}. However, in the general domain, researchers have also found other benefits to MTL beyond direct train-task performance. For example, \cite{liu2019multi} has found that MTL can be helpful as a pre-training task in natural language processing even when used across diverse, seemingly unrelated tasks, when used in conjunction with large scale autoregressive pre-training~\cite{liu2019multi}. Similarly, \todo{cite iosla}, works have also found MTL to be helpful in a pre-training/fine-tuning regime to aid in few-shot learning over natural images. \todo{look for citation for fairness and/or clustering}.

% These general domain successes have prompted significant use of MTL in the clinical domain, including \cite{harutyunyan_multitask_2017}, in which the authors examine the effect of MTL (and other strategies) on 4 benchmark tasks over MIMIC-III, finding in general MTL to be beneficial, \cite{suresh_learning_2018}, which frames predicting adverse outcomes for different patient sub-populations as a multi-task prediction problem, finding gains over predicting all populations in a single-task context, or~\cite{wu2018moleculenet}, where multi-task learning is used to predict molecular properties based on drug structures, among many other examples~\cite{wang2014multi,hunt2018multi,liu2020multi,vlachostergiou2018investigating}. 

% While these works demonstrate significant advancements using MTL in the clinical domain, they simultaneously leave many questions unanswered. For example, no works that we know of examine the possible benefits to MTL in pre-training, as has been shown helpful in the general domain~\cite{liu2019multi, iosla}. Additionally, they offer only a limited analysis of the extent of negative transfer, being focused as they are on a small set of tasks; \cite{ding2019effectiveness} examines this partially, finding that negative transfer can occur on a subset of tasks even while more rare tasks still obtain a benefit, but only within the context of ICD code prediction, and these results may not extend to other tasks.



% Here, some negative transfer is observed, but for select tasks within the molecular property prediction domain, MTL offers significant gains and appears to help especially for tasks with less training data. Numerous other examples exist, including \cite{wang2014multi,hunt2018multi,liu2020multi,vlachostergiou2018investigating}. \todo{refs review.}



% While these works represent a broad strata of use cases of MTL in the clinical domain, they simultaneously leave many important questions unanswered. Notably, these examples only offer a limited assessment on the propensity of negative transfer; \cite{ding2019effectiveness} examines this partially, finding that negative transfer can occur on a subset of tasks even while more rare tasks still obtain a benefit, but only within the context of ICD code prediction, and these results may not extend to other tasks. Further, existing works in the clinical space do not assess whether MTL offers other, representational benefits. MT-DNN~\cite{liu2019multi} shows that when trained on a broad, diverse set of input tasks, the resulting encoder yields representations capable of yielding significant performance improvements over single-task models when fine-tuned. We have no assessment of whether this is possible over clinical data, which lacks a natural analog for MT-DNN's large-scale self-supervised task. Other representation quality assessments, such as the ability of a pre-trained MTL encoder can specialize to new tasks using less training data, or better account for dataset shift, or demonstrate a strong ability to cluster, are all also open questions.

% To the best of our knowledge, prior works in this area have not yet comprehensively examined these questions, and machine learning for health lacks a full, nuanced analysis of the efficacy of MTL on clinical data and the extent of the possible drawbacks of MTL. Given that health data is notoriously noisy, sparse, and suffers from significant domain shift, this lack of understanding of MTL, one possible tool to help surmount exactly these difficulties, is a serious problem.
